A Novel Gradient Methodology with Economical Objective Function Evaluations for Data Science Applications

Gradient methods are experiencing a growth in methodological and theoretical developments owing to the challenges posed by optimization problems arising in data science. However, such gradient methods face diverging optimality gaps or exploding objective evaluations when applied to optimization problems with realistic properties for data science applications. In this work, we address this gap by developing a generic methodology that economically uses objective function evaluations in a problem-driven manner to prevent optimality gap divergence and avoid explosions in objective evaluations. Our methodology allows for a variety of step size routines and search direction strategies. Furthermore, we develop a particular, novel step size selection methodology that is well-suited to our framework. We show that our specific procedure is highly competitive with standard optimization methods on CUTEst test problems. We then show our specific procedure is highly favorable relative to standard optimization methods on a particularly tough data science problem: learning the parameters in a generalized estimating equation model. Thus, we provide a novel gradient methodology that is better suited to optimization problems from this important class of data science applications.

==> figure/catastrophic_divergence_building_function.tex <==
\begin{tikzpicture}

    % axis
    \draw[thick,->] (-.5,0) -- (8.5,0) node[anchor=north west] {$\theta$};
    \draw[thick,->] (0,-.5) -- (0,5.5) node[anchor=south east] {$f(\theta;m,1,1)$};

%    \filldraw[blue] (4,2) circle (1.5pt);
%    \filldraw[blue] (8,4) circle (1.5pt);

    % function
    \draw[thick] plot [smooth] coordinates{
        (0.0,-0.0)
(0.04020100502512563,-0.04020100502512563)
%(0.08040201005025126,-0.08040201005025126)
%(0.12060301507537688,-0.12060301507537688)
%(0.16080402010050251,-0.16080402010050251)
(0.20100502512562815,-0.20100502512562815)
%(0.24120603015075376,-0.24120603015075376)
%(0.2814070351758794,-0.2814070351758794)
%(0.32160804020100503,-0.32160804020100503)
(0.36180904522613067,-0.36180904522613067)
%(0.4020100502512563,-0.4020100502512563)
%(0.44221105527638194,-0.44221105527638194)
%(0.4824120603015075,-0.4824120603015075)
(0.5226130653266332,-0.5221017146031666)
%(0.5628140703517588,-0.5588684629176031)
%(0.6030150753768845,-0.5924029696219792)
%(0.6432160804020101,-0.622705234716295)
(0.6834170854271356,-0.6497752582005505)
%(0.7236180904522613,-0.6736130400747455)
%(0.7638190954773869,-0.6942185803388803)
%(0.8040201005025126,-0.7115918789929547)
(0.8442211055276382,-0.7257329360369688)
%(0.8844221105527639,-0.7366417514709225)
%(0.9246231155778895,-0.7443183252948158)
%(0.964824120603015,-0.7487626575086488)
(1.0050251256281406,-0.7499747481124214)
%(1.0452261306532664,-0.7479545971061337)
%(1.085427135678392,-0.7427022044897856)
%(1.1256281407035176,-0.7342175702633772)
(1.1658291457286432,-0.7225006944269085)
%(1.206030150753769,-0.7075515769803793)
%(1.2462311557788945,-0.6893702179237897)
%(1.2864321608040201,-0.66795661725714)
(1.3266331658291457,-0.6433107749804298)
%(1.3668341708542713,-0.6154326910936593)
%(1.407035175879397,-0.5843223655968283)
%(1.4472361809045227,-0.549979798489937)
(1.4874371859296482,-0.5124049897729855)
%(1.5276381909547738,-0.47220847376173314)
%(1.5678391959798996,-0.4312321097274423)
%(1.6080402010050252,-0.38959205872123315)
%(1.6482412060301508,-0.3472784340156916)
%(1.6884422110552764,-0.30428168101020203)
(1.728643216080402,-0.2605926537073424)
%(1.7688442211055277,-0.21620270123601237)
%(1.8090452261306533,-0.1711037656558081)
%(1.849246231155779,-0.12528849242758167)
%(1.8894472361809045,-0.07875035510321649)
%(1.92964824120603,-0.03148379597521744)
(1.9698492462311559,0.016515615364500746)
%(2.0100502512562812,0.06525100337542189)
%(2.050251256281407,0.11472398539117212)
%(2.090452261306533,0.16493444519395384)
%(2.130653266331658,0.21588027831082135)
%(2.170854271356784,0.26755710566494617)
(2.21105527638191,0.3199579518514699)
%(2.251256281407035,0.3730728839197808)
%(2.291457286432161,0.4268886061367243)
(2.3316582914572863,0.4813880057862896)
%(2.371859296482412,0.536549644643256)
%(2.412060301507538,0.5923471903599187)
(2.4522613065326633,0.6487487816541662)
%(2.492462311557789,0.7057163209235862)
%(2.5326633165829144,0.7632046877902945)
(2.5728643216080402,0.8211608671836848)
%(2.613065326633166,0.8795229860023608)
%(2.6532663316582914,0.9382192533125067)
%(2.693467336683417,0.9971668006427272)
(2.7336683417085426,1.0562704215034684)
%(2.7738693467336684,1.1154212131679082)
%(2.814070351758794,1.1744951295038653)
%(2.8542713567839195,1.2333514619125703)
(2.8944723618090453,1.2918312770934373)
%(2.9346733668341707,1.349755856567306)
%(2.9748743718592965,1.4069252051376175)
%(3.0150753768844223,1.463116725621249)
(3.0552763819095476,1.5180841975337684)
%(3.0954773869346734,1.5715572506612907)
%(3.1356783919597992,1.6232415935269522)
%(3.1758793969849246,1.6728203444142173)
(3.2160804020100504,1.7199569204826775)
%(3.2562814070351758,1.7643000673093767)
%(3.2964824120603016,1.8054917492854794)
%(3.3366834170854274,1.8431787507490078)
(3.3768844221105527,1.8770289162017866)
%(3.4170854271356785,1.9067529047963145)
%(3.457286432160804,1.9321320076559092)
%(3.4974874371859297,1.953051746263289)
(3.5376884422110555,1.9695393003946937)
%(3.577889447236181,1.981799902281126)
%(3.6180904522613067,1.990242918010106)
%(3.658291457286432,1.9954829029575563)
(3.698492462311558,1.9982970205337833)
%(3.7386934673366836,1.9995244397429406)
%(3.778894472361809,1.9999164886034626)
%(3.819095477386935,1.9999932309764448)
(3.85929648241206,1.9999998694574241)
%(3.899497487437186,1.9999999998930553)
%(3.9396984924623117,2.0)
%(3.979899497487437,2.0)
(4.0201005025125625,2.0)
%(4.060301507537688,2.0)
%(4.100502512562814,2.0000000001069447)
%(4.14070351758794,2.000000130542576)
(4.180904522613066,2.0000067690235555)
%(4.221105527638191,2.000083511396537)
%(4.261306532663316,2.0004755602570596)
%(4.301507537688442,2.001702979466217)
(4.341708542713568,2.0045170970424437)
%(4.381909547738694,2.009757081989894)
%(4.42211055276382,2.018200097718874)
%(4.4623115577889445,2.0304606996053063)
(4.50251256281407,2.046948253736711)
%(4.542713567839196,2.067867992344091)
%(4.582914572864322,2.0932470952036857)
%(4.623115577889448,2.122971083798214)
(4.663316582914573,2.156821249250992)
%(4.703517587939698,2.1945082507145206)
%(4.743718592964824,2.2356999326906233)
%(4.78391959798995,2.280043079517323)
(4.824120603015076,2.327179655585783)
%(4.864321608040201,2.376758406473048)
%(4.9045226130653266,2.4284427493387093)
%(4.944723618090452,2.4819158024662316)
(4.984924623115578,2.5368832743787517)
%(5.025125628140704,2.593074794862383)
%(5.065326633165829,2.6502441434326935)
%(5.105527638190955,2.7081687229065627)
(5.1457286432160805,2.7666485380874297)
%(5.185929648241206,2.8255048704961356)
%(5.226130653266332,2.8845787868320922)
%(5.266331658291457,2.943729578496531)
(5.306532663316583,3.0028331993572728)
%(5.346733668341709,3.0617807466874933)
%(5.386934673366834,3.12047701399764)
%(5.42713567839196,3.178839132816316)
(5.467336683417085,3.2367953122097046)
%(5.507537688442211,3.294283679076414)
%(5.547738693467337,3.351251218345834)
%(5.5879396984924625,3.4076528096400818)
(5.628140703517588,3.463450355356745)
%(5.668341708542713,3.5186119942137104)
%(5.708542713567839,3.5731113938632757)
%(5.748743718592965,3.6269271160802194)
(5.788944723618091,3.6800420481485308)
%(5.8291457286432165,3.7324428943350543)
%(5.869346733668341,3.784119721689178)
%(5.909547738693467,3.835065554806046)
(5.949748743718593,3.885276014608828)
%(5.989949748743719,3.9347489966245783)
%(6.030150753768845,3.9834843846354997)
%(6.07035175879397,4.031483795975218)
(6.110552763819095,4.0787503551032165)
%(6.150753768844221,4.125288492427582)
%(6.190954773869347,4.171103765655808)
%(6.231155778894473,4.216202701236012)
(6.2713567839195985,4.260592653707343)
%(6.311557788944723,4.3042816810102025)
%(6.351758793969849,4.347278434015692)
%(6.391959798994975,4.389592058721233)
(6.432160804020101,4.431232109727443)
%(6.472361809045227,4.472208473761734)
%(6.5125628140703515,4.512404989772985)
%(6.552763819095477,4.549979798489937)
(6.592964824120603,4.584322365596829)
%(6.633165829145729,4.61543269109366)
%(6.673366834170855,4.64331077498043)
%(6.71356783919598,4.66795661725714)
(6.7537688442211055,4.6893702179237895)
%(6.793969849246231,4.7075515769803795)
%(6.834170854271357,4.722500694426908)
%(6.874371859296483,4.734217570263377)
(6.914572864321608,4.7427022044897855)
%(6.954773869346734,4.747954597106133)
%(6.994974874371859,4.749974748112422)
%(7.035175879396985,4.748762657508649)
(7.075376884422111,4.744318325294816)
%(7.115577889447236,4.7366417514709225)
%(7.155778894472362,4.725732936036969)
%(7.1959798994974875,4.711591878992954)
(7.236180904522613,4.69421858033888)
%(7.276381909547739,4.673613040074746)
%(7.316582914572864,4.649775258200551)
%(7.35678391959799,4.622705234716295)
(7.396984924623116,4.592402969621979)
%(7.437185929648241,4.558868462917603)
%(7.477386934673367,4.522101714603166)
%(7.517587939698492,4.482412060301508)
(7.557788944723618,4.442211055276382)
%(7.597989949748744,4.402010050251256)
%(7.63819095477387,4.36180904522613)
%(7.678391959798995,4.321608040201005)
(7.71859296482412,4.28140703517588)
%(7.758793969849246,4.241206030150754)
%(7.798994974874372,4.201005025125628)
%(7.839195979899498,4.160804020100502)
(7.8793969849246235,4.1206030150753765)
%(7.919597989949749,4.080402010050251)
%(7.959798994974874,4.040201005025126)
(8.0,4.0)
    };

\end{tikzpicture}

==> section/abstract.tex <==
Gradient methods are experiencing a growth in methodological and theoretical developments owing to the challenges of optimization problems arising in data science.
Focusing on data science applications with expensive objective function evaluations yet inexpensive gradient function evaluations, gradient methods that never make objective function evaluations are either being rejuvenated or actively developed. 
However, as we show, such gradient methods are all susceptible to catastrophic divergence under realistic conditions for data science applications.
In light of this, gradient methods which make use of objective function evaluations become more appealing, yet, as we show, can result in an exponential increase in objective evaluations between accepted iterates.
As a result, existing gradient methods are poorly suited to the needs of optimization problems arising from data science.
In this work, we address this gap by developing a generic methodology that economically uses objective function evaluations in a problem-driven manner to prevent catastrophic divergence and avoid an explosion in objective evaluations between accepted iterates. 
Our methodology allows for specific procedures that can make use of specific step size selection methodologies or search direction strategies, and we develop a novel step size selection methodology that is well-suited to data science applications.
We show that a procedure resulting from our methodology is highly competitive with standard optimization methods on CUTEst test problems.
We then show a procedure resulting from our methodology is highly favorable relative to standard optimization methods on optimization problems arising in our target data science applications. 
Thus, we provide a novel gradient methodology that is better suited to optimization problems arising in data science.


==> section/algo_psuedocode/inner_loop.tex <==
\begin{algorithm}
    \caption{Modified Gradient Descent with Triggering Events}
    \label{alg:inner loop}
    \begin{algorithmic}[1]
    \Procedure{ModifiedGD}{$\nabla F, \hat{L}_{i, 0}, \delta_{(i, \cdot)}, R, \theta_{i, 0}, \kappa_{(i,\cdot)}, T^*, \ell, \gamma$}
    
        % run steepest descent
        %------------------------------------------
        \State $ \Delta \leftarrow 0 $ \Comment{Measure of predicted decrease of objective}
        \For{$j = 0, 1, ..., T^*-1$}
        \State $\alpha_{i,j} \leftarrow \delta_{(i,\cdot)} (2||\nabla F(\theta_{i,j})||^3 + ||\nabla F(\theta_{i,j})||^2\hat{L}_{i,j} )^{-1}$ \Comment{Step size computation}
        \State $\theta_{i, j+1} \leftarrow \theta_{i,j} - \alpha_{i,j} \nabla F(\theta_{i,j})$ \Comment{Gradient step}
        \State $\Delta \leftarrow \Delta - \delta_{(i,\cdot)}^2\left( 4||\nabla F(\theta_{i,j})||^3 + 2\hat{L}_{i,j}||\nabla F(\theta_{i,j}) ||^2 \right)^{-1}$ \Comment{Update predicted decrease}
        \If{ $|| \theta_{i,j} - \theta_{i,j+1} || \ge 10^{-10}$ }
            \State $\hat{L}_{i,j+1} \leftarrow \Call{UpdateL}{\nabla F, \theta_{i,j}, \theta_{i,j+1}, \hat{L}_{i,j}, \kappa_{(i,\cdot)}, \ell}$ \Comment{Update local Lipschitz estimate}
        \Else
            \State $\hat{L}_{i,j+1} \leftarrow \hat{L}_{i,j}$
        \EndIf
        \State $ \delta_{cond} \leftarrow ||\nabla F(\theta_{i,j+1})||^2 \not\in (\delta_{(i,\cdot)}, \gamma\delta_{(i,\cdot)})$ 
        \If{$\delta_{cond}$ or $||\theta_{i,j+1}-\theta_{i,0}|| > R$ or stop condition} \Comment{Check triggering events}
        \State \Return{$\theta_{i,j+1},\hat{L}_{i,j+1},\delta_{cond},\Delta$}
        \EndIf
        
        \EndFor
        \State
        \Return{$\theta_{i,T^*},\hat{L}_{i,T^*},\delta_{cond},\Delta$}
        %------------------------------------------
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> section/algo_psuedocode/naive_algorithm.tex <==
\begin{algorithm}[ht]
    \caption{An Example Procedure of Our Method}
    \label{alg-naive-algorithm}
    \begin{algorithmic}[1]
    \Require $F, \dot F, \theta_{0}, \epsilon > 0$
        
    % Step Size 
    \State $\delta \leftarrow 1$ \Comment{Step size}
    
    % Outer Loop Counter
    \State $k \leftarrow 0$ \Comment{Outer Loop Counter}
    
    % Objective Function Value
    \State $\tau_{\obj} \leftarrow F(\theta_0)$ \Comment{Reference for objective function value}
    
    
    % Outer Loop
    \While{$\inlinenorm{ \dot F(\theta_k) } > \epsilon$} \Comment{Outer Loop}
    
    % Inner Loop Counter
    \State $j, \psi_0 \leftarrow 0, \theta_k$ \Comment{Inner Loop Initialization}
    
    % Thresholds and Tests
    \State $\tau_{\iter,\exit},~\tau_{\iter,\max} \leftarrow 3\inlinenorm{\dot F(\theta_k)}_2, 100$ \Comment{Test thresholds on iterates}
    \State $\tau_{\gra,\low},~\tau_{\gra,\upp} \leftarrow 0.5\inlinenorm{\dot F(\theta_k)}_2, 1.5\inlinenorm{ \dot F(\theta_k)}_2$ 
    \Comment{Test thresholds on gradient}
    
    % Inner Loop
    \While{$\true$} \Comment{Inner Loop}
    
    		%Check if in the exit or growth in gradient
    		\If{ $\inlinenorm{ \psi_j - \theta_k }_2 > \tau_{\iter,\exit}$ 
    			\textbf{or} $\inlinenorm{ \dot F(\psi_j)}_2 \not\in (\tau_{\gra,\low}, \tau_{\gra,\upp})$ 
    			\textbf{or} $j == \tau_{\iter,\max}$} 
    			\If{ $F(\psi_j) \geq \tau_{\obj} - 10^{-3} \delta \inlinenorm{ \dot F(\theta_k)}_2^2 $ }
    				\State $\theta_{k+1}, \delta, k \leftarrow \theta_k, 0.5 \delta, k+1$
    				\Comment{Reset iterate with reduced step size}
    			\ElsIf{ $\inlinenorm{ \dot F(\psi_j)}_2 \leq \tau_{\gra,\low}$ }
    				\State $\theta_{k+1}, k, \tau_{\obj} \leftarrow \psi_j, k+1, F(\psi_j)$
				\Comment{Accept iterate and leave step size unchanged}    			
    			\Else
    				\State $\theta_{k+1}, \delta, k, \tau_{\obj} \leftarrow \psi_j, 1.5\delta, k+1, F(\psi_j)$
    				\Comment{Accept iterate and increase step size}
    			\EndIf
    			\State Exit Inner Loop
    		\EndIf
    		
    		\State $\psi_{j+1}, j \leftarrow \psi_j - \delta \dot F(\psi_j), j+1$
    		\Comment{Standard gradient method}
    
    \EndWhile %End inner loop
    
    
    \EndWhile %End Outer Loop
	\State \Return $\theta_k$    
    \end{algorithmic}
    
\end{algorithm} 

==> section/algo_psuedocode/outer_loop.tex <==
\begin{algorithm}[]
    \caption{Gradient Descent with Stopping Times for Step Size Selection}
    \label{alg:outer loop}
    \begin{algorithmic}[1]
    \Require $F, \nabla F, R, \theta_{0,0}, \kappa_{(0,\cdot)}, T^*, \ell, \gamma, c_1 (\in (0,1])$ 
    
    \Procedure{Initialization}{ $\nabla F, \theta_{0,0}$ }
    \State\Return{ $(||\nabla F(\theta_{0, 0} + \epsilon)-\nabla F(\theta_{0,0})||)(||\epsilon||^{-1})$ } \Comment{Random perturbation to form estimate}
    \EndProcedure
    
    % outer loop
    \State $\delta_{cond} \leftarrow True$ \Comment{ Represent when we need to change $\delta_{(i,\cdot)}$ }
    \State $\hat{L}_{0,0} \leftarrow \min(1, \Call{Initialization}{\nabla F, \theta_{0,0}}) + \ell$ \Comment{ Initial local Lipschitz estimate}
    \State $c_2 = \frac{2 + \sqrt{4-4c_1}}{2}$ \Comment{ Factor for increasing step size }
    \For{$i = 0,1,...$} \Comment{Outer loop}
    
    % Do we accept the new point
    %------------------------------------------
    \If{$\delta_{cond}$} \Comment{Initialization of gradient lower bound}
        \State $\delta_{(i, \cdot)} \leftarrow ||\nabla F(\theta_{i, 0})||^2/2$
    \EndIf
    %------------------------------------------
    
    \State $\theta_{i, T_i}, \hat{L}_{i, T_i}, \delta_{cond}, \Delta \leftarrow \Call{ModifiedGD}{\nabla F, \hat{L}_{i, 0}, \delta_{(i, \cdot)}, R, \theta_{i, 0}, \kappa_{(i,\cdot)}, T^*, \ell, \gamma}$ \Comment{ Inner loop}
    \If{stop condition}
        \State \Return $\theta_{i, T_i}$
    \EndIf
    
    \If{$F(\theta_{i, T_i}) - F(\theta_{i, 0}) > c_1\Delta$} \Comment{Check if we sufficiently decreased the objective}
    \State $\hat{L}_{i+1, 0} \leftarrow 2\hat{L}_{i, T_i} $  \Comment{Inflation to meet descent criterion}
    \State $\kappa_{(i+1,\cdot)} \leftarrow 1$ \Comment{Stop decreasing local Lipschitz estimate in ModifiedGD}
    \State $\theta_{i+1, 0} = \theta_{i, 0}$ \Comment{Restart from previous point}
    \State $\delta_{(i+1,\cdot)} = \delta_{(i,\cdot)}$
    \State $\delta_{cond} = False$
    \Else \Comment{ Accept this iterate and continue }
    \State $\theta_{i+1, 0} \leftarrow \theta_{i, T_i}$
    \State $\kappa_{(i+1,\cdot)} \leftarrow \kappa_{0,\cdot}$
    \EndIf
    
    \EndFor
    \end{algorithmic}
    
    \end{algorithm} 

==> section/algorithm_intuition.tex <==
\input{section/algo_psuedocode/naive_algorithm.tex}

We will begin by discussing the standard gradient method. We will then reason about the short-term behavior of this gradient method in order to introduce a specific case of our procedure. Specifically, we will use our reasoning about the short-term behavior of the gradient method to introduce inexpensive tests. When the tests are triggered (i.e., are evaluated as true), we will evaluate the objective function at this triggering iterate and modify the standard gradient method based on this information.

Consider an initial point, $\theta_0 \in \mathbb{R}^n$. Then, the standard gradient method generates a sequence, $\lbrace \theta_k : k\in\mathbb{N} \rbrace$, according to
\begin{equation}
\theta_{k} = \theta_{k-1} - \alpha \dot F(\theta_{k-1}), ~ k \in \mathbb{N}.
\end{equation}
This gradient method's iterates may eventually converge to a solution, oscillate in a cycle, approach a limit cycle, or diverge. While this asymptotic iterate behavior is important, the short-term iterate behavior is what we need to reason about to build our algorithm. The short-term iterate behavior can be reasoned about by imagining two constructions: a closed ball centered at $\theta_0$ of arbitrary, finite radius; and a positive open interval containing $\inlinenorm{ \dot F(\theta_0)}_2$. Then, trivially, the iterates will either exit, or remain inside, the ball; and the iterates' gradient norms will either exit, or remain inside, the interval containing $\inlinenorm{ \dot F(\theta_0)}_2$.

Based on these trivial constructions and the behavior of the iterates relative to them, our gradient algorithm tests them at each iteration. Specifically, at each iterate, our algorithm tests:
\begin{remunerate}
\item Has the iterate exited the closed ball around $\theta_0$?
\item Has the iterate's gradient norm escaped the interval containing $\inlinenorm{ \dot F(\theta_0)}_2$?
\item If the iterate has not exited the closed ball around $\theta_0$ and its gradient norm has remained in the interval containing $\inlinenorm{ \dot F(\theta_0)}_2$, has it been a ``long time'' since any of the above situations occurred?
\end{remunerate}
If any of the above situations comes back as being true at a given iterate, then our algorithm checks whether the objective function value has decreased sufficiently at the triggering iterate relative to the reference value, $F(\theta_0)$. If the objective function value at the triggering iterate has not sufficiently decreased, then we are concerned about non-convergence and we address this by restarting the procedure at $\theta_0$ and scale the step size down. If the objective function value at the triggering iterate has decreased relative to $F(\theta_0)$, then we suspect that this iterate is closer to a solution than $\theta_0$. In this case, we will shift the closed ball around the triggering iterate, shift the interval to be positive and contain the gradient-norm of the triggering iterate, and we will take the objective function value at this triggering iterate as our new reference value. Moreover, we can adjust the step size as well. For example, if we observe that the gradient norm has dropped below the interval at the triggering iterate, then we might conservatively keep the step size the same. If we observe that the gradient norm has not dropped below the interval at the triggering iterate, then we might choose to increase the step size to take advantage of large gradient values to make more progress.

As a specific example of our method, the above procedure is formalized in \Cref{alg-naive-algorithm} with supplied example values for the radius of the closed ball, $\tau_{\iter,\exit}$; the gradient-norm interval $(\tau_{\gra,\low},\tau_{\gra,\upp})$; and the number of iterates since a triggering iterate, $\tau_{\iter,\max}$. The procedure in \Cref{alg-naive-algorithm} differs from the above description as it is reorganized into an inner loop---the iterates between positive tests---and an outer loop---the iterates whenever a positive test is triggered.

By examining \Cref{alg-naive-algorithm}, our procedure has two important properties (which we formalize later). First, our procedure guarantees $F(\theta_k) \leq F(\theta_0)$ for all $k \in \mathbb{N}$. Hence, our procedure cannot experience the catastrophic divergence that is endemic to objective-function-evaluation-free methods (see \Cref{table-objective-free}). Second, by \Cref{as-loc-lip-cont} and the use of a fixed ball around the current iterate, our procedure must produce an outer loop iterate distinct from previous iterates with a finite worst-case number of objective function evaluations. Moreover, this number can only increase multiplicatively between two distinct iterates if the local Lipschitz constant of the gradient function is decaying multiplicatively. In turn, the iterates are entering a shallow region of the objective function, which will rapidly trigger the overall stopping condition for the outer loop. As a result, our procedure hedges against the exponentially increasing number of objective evaluations that can plague the methods in \Cref{table-multiple-objective-evaluation}.

==> section/notation.tex <==
\begin{table}[!ht]
    \centering
    \caption{Notation for Algorithm}
    \begin{tabular}{p{5cm} p{9cm}}
        \toprule
        $F(\theta), \dot{F}(\theta), \ddot{F}(\theta)$ & Objective, gradient of objective, and Hessian of objective, respectively.\\
        $k,j$ & Outer and inner loop iteration counters. \\
        $\theta_k$ & $k$th outer loop iterate. \\
        $\psi_j^k$ & $j$th inner loop iterate for outer loop iteration $k$.\\
        $\tau^k_{\iter,\exit}$ & Radius for bounding ball triggering event.\\
        $\tau^k_{\iter,\max}$ & Maximum inner loop iteration allowance.\\
        $\tau^k_{\gra,\upp}, \tau^k_{\gra,\low}$ & Upper and lower thresholds for gradient triggering event.\\
        $\delta, \delta_k$ & Step size scaling term.\\
        $\tau^k_{\obj}$ & Nonmonotone search threshold.\\
        $w$ & Number of objective values in nonmonotone search.\\
        $\rho$ & Relaxation term in nonmonotone Armijo condition.\\
        $\sigma_{\upp}, \sigma_{\low}$ & Inflation and Reduction factors for step size scaling term.\\
        $\alpha, \alpha_j^k, \mathrm{StepSize}$ & Step size, and the function that produces the step size.\\
        $\gamma, \gamma_j^k, \mathrm{StepDirection}$ & Step applied to each inner loop iterate, and the function that produces the step.\\
        $\epsilon$ & Gradient threshold for termination.\\
        $\hat{L}_j^k$ & Approximation of local Lipschitz constant\\\bottomrule
    \end{tabular}
\end{table}

\begin{table}[!ht]
    \centering
    \caption{Notation for Theory}
    \begin{tabular}{p{5cm} p{9cm}}
        \toprule
        $\mathbb{N}, \mathbb{R}^n$ & Natural numbers, n-dimensional Euclidean space.\\
        $\inlinenorm{\cdot}_2$ & Euclidean norm. \\
        $C, C_k, C_u'$ & Compact sets. \\
        $\underline g(C)$ & Constant in compact set $C$ to ensure step direction is a descent direction. See \cref{property-stepdirection-negative}. \\
        $\overline g(C)$ & Constant in compact set $C$ to ensure the norm of step direction is within some factor of the norm gradient. See \cref{property-stepdirection-propgrad}. \\
        $\overline \alpha(C)$ & Upper bound on step size in compact set $C$. See \cref{property-stepsize-upper}. \\
        $\underline \alpha(C)$ & Lower bound on step size in compact set $C$. See \cref{property-stepsize-lower}.\\
        $\overline \tau_{\exit}(\theta)$ & Upper bound on radius for bounding ball. See \cref{property-radius-bounded}.\\
        $\overline \tau_{\max}$ & Upper bound on maximum number of inner loop iterations. See \cref{property-iter-max}.\\
        $\mathcal{B}(\theta), \mathcal{B}(\theta, R)$ & Ball around $\theta$. Radius either specified implicitly or with $R$.\\
        $\mathcal{G}(\theta), \mathcal{G}(\theta, R)$ & Max norm gradient within the ball $\mathcal{B}(\theta)$ or $\mathcal{B}(\theta, R)$.\\
        $\mathcal{L}(C)$ & Local Lipschitz constant within compact set $C$.\\
        $\ell_k$ & Index of iterates that satisfied the nonmonotone Armijo Condition.\\
        $L(k)$ & Sub-index of last accepted iterate.\\
        $O(k)$ & Largest sub-index smaller than $L(k)$ such that $\ell_{O(k)}$ is the index of the iterate, whose objective value is used as the nonmonotone threshold.\\
        $o_s$ & Sub-index such that $\ell_{o_s}$ are the indices of the iterates, whose objective values are used as nonmonotone thresholds.\\
        $g_u$ & Subindices for $\ell$ of distinct iterates used in analysis of the gradient.\\\bottomrule
    \end{tabular}
\end{table}

==> table/data_science_problems_table.tex <==
\begin{table}[hb]
\centering
\caption{Below are canonical data science problems, a reference for the problem, and different smoothness conditions: globally Lipschitz smooth (GRA); globally Lipschitz Hessian smooth (HES); subquadratically Lipschitz smooth (SUB); quadratically Lipschitz smooth (QUA); and local Lipschitz continuity of the gradient (LOC). See \cref{subsec:smoothness-overview} for definitions. We indicate ``yes'' if the problem satisfies the condition and ``no'' if not. Details can be found in the indicated section.}
\label{table-data-science-problems}
\footnotesize
\begin{tabular}{@{}>{\raggedright}p{1.5in}lllllll@{}} \toprule
\textbf{Problem} & \textbf{Ref.} & \textbf{GRA} & \textbf{HES} & \textbf{SUB} & \textbf{QUA} & \textbf{LOC} & \textbf{Details} \\ \midrule
Factor Analysis for Pattern Extraction & \cite[\S 4]{lawley1962factor} & No & No & No & Yes & Yes & \Cref{subsec:factor-analysis}\\
Classification via Feed Forward Neural Network & \cite[Chapter 8]{rumelhart1987} & No & No & No & Yes & Yes & \Cref{subsec:classification-nn}\\
%Poisson Regression Model for Count Data & \cite[Chapter 6]{mccullagh1989glm} & No & No & No & Yes & \Cref{subsec:poisson-reg}\\
Correlation Modeling via Generalized Estimating Equations & \cite[Chapter 3]{lipsitz2008geelongitudinal} & No & No & No & Yes & Yes & \Cref{subsec:gee}\\\bottomrule
\end{tabular}
\end{table}

==> table/multiple_objective_evaluation_table.tex <==
\begin{table}[ht]
\centering
\caption{Gradient methods that may use multiple objective function evaluations per accepted iterate. For each method, a short description, a convergence result reference, and an exploding evaluation example are given.}
\label{table-multiple-objective-evaluation}
\footnotesize
\begin{tabular}{@{}>{\raggedright}p{1.5in}>{\raggedright}p{2.5in}l@{}} \toprule
\textbf{Method} & \textbf{Convergence} & \textbf{Exploding Evaluations} \\ \midrule
Armijo's Backtracking Method & \cite[Corollary 2]{armijo1966minimization}, \cite[Theorem 5]{zhang2020firstorder} & \Cref{subsec:armijo-backtracking}\\
Newton's Method with Cubic Regularization & \cite[Theorem 1]{nesterov2006cubic} & \Cref{subsec:cubic-newton-method}\\
Lipschitz Constant(s) Line Search Methods & \cite[Theorem 3]{nesterov2012GradientMF}, \cite[Theorem 2]{curtis2018exploiting} & \Cref{subsec:lipschitz-line-search}\\
Adaptive Cubic Regularization &  \cite[Theorem 2.5]{cartis2011cubic1}, \cite[Theorem 2.1]{cartis2011cubic2} & \Cref{subsec:adaptive-cubic-reg}\\
%Nonconvex Bregman Distance Method & \cite[Theorem 4.1]{bolte2018first} & \\ 
\bottomrule
\end{tabular}
\end{table}

==> table/novel-step-size-param-table.tex <==
\begin{table}[hb]
    \centering
    \caption{Example of a parameter set that works well with \cref{alg:novel-step-size} and satisfies the necessary properties. }
    \label{table:novel-step-size-parameters}
    \footnotesize
    \begin{tabular}{llllllll@{}} \toprule
    \textbf{Parameter} & $\hat{L}_{l.b.}$ & $\tau^k_{\gra,\low}$ & $\tau^k_{\gra,\upp}$ & $\tau^k_{\iter,\exit}$ & $\tau^k_{\iter, \max}$ & $\sigma_{\upp}$ & $\sigma_{\low}$ \\ \midrule
    \textbf{Value} & $10^{-10}$ & $\inlinenorm{\dot{F}(\theta_k)}/\sqrt{2}$ & $\sqrt{20}\tau^k_{\gra,\low}$ & $10$ & $100$ & $1.1$ & $.5$  \\\bottomrule
    \end{tabular}
\end{table}

==> table/objective_free_table.tex <==
\begin{table}[ht]
\centering
\caption{Gradient methods that do not use objective function information. The method, convergence result reference(s), and a reference to a catastrophic divergence example are listed.}
\label{table-objective-free}
\footnotesize
\begin{tabular}{@{}>{\raggedright}p{1.5in}>{\raggedright}p{2.5in}l@{}} \toprule
\textbf{Method} & \textbf{Convergence} & \textbf{Divergence} \\ \midrule
Diminishing Step-Size & \cite[Proposition 1.2.4]{bertsekas1999}, \cite[Theorem 3.7]{patel2023gradient} & \cite[Proposition 4.4]{patel2023gradient} \\
Constant Step-Size & \cite[Corollary 1]{armijo1966minimization}, \cite[Theorem 3]{zhang2020gradientclipping}, \cite[Theorem 5.1]{li2023convex} & \Cref{subsec:ce-constant} \\
Barzilai-Borwein Methods & \cite[\S 4]{barzilai1988}, \cite[Theorem 3.3]{burdakov2019stabilized} & \Cref{subsec:ce-bbb} \\
Nesterov's Acceleration Method & \cite[Theorem 6]{nesterov2012GradientMF}, \cite[Theorem 4.4]{li2023convex} & \Cref{subsec:ce-nag} \\
Bregman Distance Method & \cite[Theorem 1]{bauschke2017descentlemma}	&  \Cref{subsec:ce-bregman}\\
Negative Curvature Method & \cite[Theorem 1]{curtis2018exploiting} & \Cref{subsec:ce-negative}\\
Lipschitz Approximation & \cite[Theorem 1]{malitsky2020adaptive} & \Cref{subsec:ce-lipschitz}\\
Weighted Gradient-Norm Damping & \cite[Theorem 2.3]{wu2020wngrad}, \cite[Corollary 1]{grapiglia2022AdaptiveTrust} & \Cref{subsec:ce-weighted}\\
Adaptively Scaled Trust Region & \cite[Corollary 3.3]{gratton2022firstorderOFFO}, \cite[Theorem 3.10]{gratton2022firstorderOFFO}, \cite[Theorem 3.3]{gratton2023OFFOSecondOrderOpt} & \Cref{subsec:ce-adaptiveTR}\\ \bottomrule
\end{tabular}
\end{table}
